Information Seeking for Robust Decision Making under Partial Observability

Explicit information seeking is essential to human problem-solving in practical environments characterized by incomplete information and noisy dynamics. When the true environmental state is not directly observable, humans seek information to update their internal dynamics and inform future decision-making. Although existing Large Language Model (LLM) planning agents have addressed observational uncertainty, they often overlook discrepancies between their internal dynamics and the actual environment. We introduce Information Seeking Decision Planner (InfoSeeker), an LLM decision-making framework that integrates task-oriented planning with information seeking to align internal dynamics and make optimal decisions under uncertainty in both agent observations and environmental dynamics. InfoSeeker prompts an LLM to actively gather information by planning actions to validate its understanding, detect environmental changes, or test hypotheses before generating or revising task-oriented plans. To evaluate InfoSeeker, we introduce a novel benchmark suite featuring partially observable environments with incomplete observations and uncertain dynamics. Experiments demonstrate that InfoSeeker achieves a 74% absolute performance gain over prior methods without sacrificing sample efficiency. Moreover, InfoSeeker generalizes across LLMs and outperforms baselines on established benchmarks such as robotic manipulation and web navigation. These findings underscore the importance of tightly integrating planning and information seeking for robust behavior in partially observable environments. The project page is available at https://infoseekerllm.github.io

==> 9_statements.tex <==
\section*{Reproducibility Statement}
\label{reproducibility}
The complete implementation of our proposed \method{} along with the benchmarks is included in the supplementary material. While the implementations of baseline methods and ablation experiments are not included, we provide the corresponding prompts used with LLMs in Appendix~\ref{prompts}.

==> src/equations/world_model.tex <==
\begin{equation}
M^{\text{LLM}} = (S^{\text{LLM}}, A, Z^{\text{LLM}}, T^{\text{LLM}}, O^{\text{LLM}}, R, \gamma^{\text{LLM}})
\label{eq:world_model}
\end{equation}

==> src/tables/llm3.tex <==
\begin{table}[H]
    \centering
    \tb{@{}l|ccc|ccc@{}}{1.0}{
        & \multicolumn{3}{c}{Setting 1} & \multicolumn{3}{|c}{Setting 2}\\
        \cmidrule{2-7}
        & Easy & Medium & Hard & Small & Medium & Large\\
        \midrule
        %\textit{GPT 4} & & & & & &  \\        
        %\hspace{0.2cm} LLM3 (backtrack) & \textbf{100} & \textbf{100} & 60 & 60 & \textbf{80} & 50\\
        %\hspace{0.2cm} LLM3 (from scratch) & \textbf{100} & \textbf{100} & \textbf{70} & \textbf{70} & 70 & %\textbf{60}\\
        %\midrule
        %\midrule
        %\textit{GPT 4o} & & & & & & \\    
        LLM3 (backtrack) & \textbf{100} & 80 & 50 & 50 & 80 & 50\\
        LLM3 (from scratch) & \textbf{100} & \textbf{100} & \textbf{80} & \textbf{80} & 90 & 60\\
        \method{} (ours) & \textbf{100} & \textbf{100} & 70 & 70 & \textbf{100} & \textbf{80}\\
        \bottomrule
    }
    \vspace{10pt}
    \caption{\textbf{LLM3 benchmark~\ref{wang2024llm3}.} This benchmark requires agents to control a robotic arm to pack objects into a basket in a simulated environment. In Setting 1, all baskets are fully reachable, with difficulty increasing by object volume. In Setting 2, object size is fixed at the most challenging level, and larger baskets reduce reachable areas.}
    \label{tab:llm3}
\end{table}

==> src/tables/travelplanner.tex <==
\begin{table}[H]
    \centering
    \tb{@{}l|c@{}}{1.0}{
         & Final Pass Rate (↑) \\
        \midrule
        ReAct (using original prompt) & 5.56 \\
        LLM3 (backtrack)              & 5.00 \\
        LLM3 (from scratch)           & 5.56 \\
        \method{} (ours)    & \textbf{6.11} \\
    }
    \vspace{10pt}
    \caption{\textbf{TravelPlanner benchmark~\ref{xie2024travelplanner}.} This benchmark evaluates web agents on their ability to gather user-specific information and generate valid travel plans. All methods are evaluated with a fixed 100-step interaction limit for consistency with Tab.~\ref{tab:results}.}
    \label{tab:travelplanner}
\end{table}

==> src/tables/uncertain.tex <==
\begin{table}[ht]
    \centering
    \tb{@{}l|cc@{}}{1.0}{
        & basic & perturbed \\
        \midrule
        %\textit{Original} & & \\
        %\hspace{0.2cm} ReAct & 68 & 22 \\
        %\hspace{0.2cm} AdaPlanner & 14 & 0 \\
        %\hspace{0.2cm} LLM3 (backtrack) & 76 & 6 \\
        %\hspace{0.2cm} LLM3 (from scratch) & 86 & 0 \\
        \textit{With Uncerntain Prompt} & & \\
        \hspace{0.2cm} ReAct & 62 & 28 \\
        \hspace{0.2cm} AdaPlanner & 8 & 4 \\
        \hspace{0.2cm} LLM3 (backtrack) & 80 & 12 \\
        \hspace{0.2cm} LLM3 (from scratch) & \textbf{90} & 12 \\
        \midrule
        \method{} (ours) & 82 & \textbf{62} \\
        \bottomrule
    }
    \caption{\textbf{Explicit uncertainty in prompts yields minimal gains.} On the \textit{stack single block} task, adding uncertainty descriptions to baseline prompts results in only marginal improvement. This highlights the limitations of prompting alone and the necessity of explicit information-seeking.}
    \label{tab:uncertain}
\end{table}

==> src/tables/wall_clock.tex <==
\begin{table}[H]
    \centering
    \tb{@{}l|cc@{}}{1.0}{
        & basic & perturbed \\
        \midrule
        ReAct & 68 & 30 \\
        AdaPlanner & 10 & 0 \\
        LLM3 (backtrack) & 98 & 46 \\
        LLM3 (from scratch) & 98 & 62 \\
        \method{} (ours) & \textbf{100} & \textbf{98} \\
        \bottomrule
    }
   \caption{\textbf{Time efficiency of \method{}.} We evaluate all methods on the \textit{stack single block} task, with a fixed wall-clock time budget of 1 minute per trial. \method{} demonstrates the highest efficiency, achieving a $36\%$ performance improvement over the previous state-of-the-art, LLM3.}
   \label{tab:wall_clock}
\end{table}
